Normalise or condition? Noise-floor front-ends for on-board keyword spotting under UAV rotor ego-noise

A microphone on the airframe of a small multi-rotor UAV is dominated by rotor ego-noise, so spoken flight commands arrive at negative signal-to-noise ratio (SNR). We study small-footprint keyword spotting (KWS) for a ten-word command vocabulary under real ego-noise, training on one quadrotor and testing on another. Besides per-clip accuracy we measure the streaming false-alarm rate on 4.4 h of continuous rotor noise. We compare classical noise-robust front-ends (CMN, PCEN, spectral subtraction), test-time adaptation, and two front-ends that track the per-band ego-noise floor over the two seconds preceding the decision window and either subtract it (normalisation) or feed it to the network as a second input channel (conditioning). Per clip, all front-ends look alike: +2-3 points on average, up to +14 at -15 dB. On continuous rotor noise they differ sharply. Normalising front-ends fire about ten times more often than plain log-mel at the same threshold and end up below it at a budget of one false alarm per hour (-9 points at 0 dB). Conditioning keeps the baseline's false-alarm rate and turns its gain into detections (+8 points at -10 dB over three seeds); on top of PCEN it gives the best per-clip accuracy and false-alarm rate, and a level-anchored variant is also invariant to the microphone gain. Real drone+interferer recordings expose the remaining failure mode, environmental sounds and bystander speech, which training negatives halve. A single script reproduces all on-device numbers on the NVIDIA Jetson Orin NX flight computer, where the complete pipeline costs 3 ms per 100 ms hop on the CPU.

==> tables/ablation.tex <==
20th pct., 2\,s, speech in ctx (default) & 83.0 & 52.3 & 89.7 & 7.3 \\
5th percentile & 81.8 & 49.5 & 89.1 & 10.4 \\
50th percentile & 83.8 & 55.3 & 90.2 & 7.0 \\
mean & 84.2 & 52.6 & 90.9 & 0.6 \\
0.5\,s context & 82.7 & 52.0 & 89.5 & 7.3 \\
no speech in training context & 82.8 & 52.5 & 89.5 & 9.8 \\%


==> tables/gain.tex <==
BC-ResNet-8 & log-mel & 83.4 & 88.8 & 90.0 & 88.9 & 87.3 \\
BC-ResNet-8 & CMN & 89.8 & 89.8 & 89.8 & 89.8 & 89.8 \\
BC-ResNet-8 & PCEN & 89.7 & 89.7 & 89.8 & 89.6 & 89.7 \\
BC-ResNet-8 & \nfn & 90.2 & 90.2 & 90.2 & 90.2 & 90.2 \\
BC-ResNet-8 & \npc & 83.4 & 89.6 & 90.3 & 89.9 & 89.4 \\
BC-ResNet-8 & \npca & 90.9 & 90.9 & 90.9 & 90.9 & 90.9 \\
BC-ResNet-3 & log-mel & 59.2 & 83.1 & 86.3 & 85.2 & 82.3 \\
BC-ResNet-3 & \nfn & 85.5 & 85.5 & 85.5 & 85.5 & 85.5 \\
BC-ResNet-3 & \npca & 87.2 & 87.2 & 87.3 & 87.3 & 87.3 \\%


==> tables/models.tex <==
BC-ResNet-3 & 57\,k & 75.9 & 78.9 & 77.7 & 79.2 & 2.5 & 5.0 & 5.0 & 2.0 \\
BC-ResNet-3 FiLM & 66\,k & -- & -- & -- & 75.6 & -- & -- & -- & 5.0 \\
BC-ResNet-8 & 349\,k & 81.3 & 83.0 & 83.3 & 84.0 & 6.2 & 7.3 & 2.8 & 2.2 \\
BC-ResNet-8 FiLM & 368\,k & -- & -- & -- & 81.0 & -- & -- & -- & 5.0 \\
KWT-1 & 558\,k & 61.9 & 68.8 & 62.6 & -- & 2.2 & 4.5 & 0.6 & -- \\%


==> tables/streaming.tex <==
BC-ResNet-8 log-mel$^{\dagger}$ & 51.7\,$\pm$\,1.6 & 75.0\,$\pm$\,0.9 & 84.2\,$\pm$\,1.5 & 89.8\,$\pm$\,1.1 \\
BC-ResNet-8 CMN & 44.5 & 63.5 & 74.9 & 78.6 \\
BC-ResNet-8 PCEN & 56.5 & 75.2 & 82.6 & 88.2 \\
BC-ResNet-8 \nfn$^{\dagger}$ & 46.4\,$\pm$\,1.7 & 64.9\,$\pm$\,2.1 & 75.3\,$\pm$\,0.8 & 81.9\,$\pm$\,1.1 \\
BC-ResNet-8 \npc$^{\dagger}$ & 58.5\,$\pm$\,3.4 & 74.9\,$\pm$\,2.6 & 84.9\,$\pm$\,2.3 & 89.7\,$\pm$\,2.7 \\
BC-ResNet-8 \npca$^{\dagger}$ & 59.7\,$\pm$\,1.8 & 75.9\,$\pm$\,1.5 & 85.5\,$\pm$\,0.5 & 91.1\,$\pm$\,0.3 \\
BC-ResNet-8 PCEN+\npca$^{\dagger}$ & 60.8\,$\pm$\,3.2 & 78.0\,$\pm$\,1.0 & 84.6\,$\pm$\,0.9 & 89.7\,$\pm$\,1.1 \\
BC-ResNet-3 log-mel & 47.0 & 75.7 & 83.3 & 88.5 \\
BC-ResNet-3 \nfn & 44.8 & 64.2 & 72.1 & 79.5 \\
BC-ResNet-3 \npca & 55.0 & 75.0 & 85.4 & 89.2 \\%


==> tables/tta.tex <==
log-mel & 81.7$\rightarrow$81.3 & 44.4$\rightarrow$44.6 \\
\nfn & 83.3$\rightarrow$82.2 & 53.3$\rightarrow$48.7 \\
\npc & 83.5$\rightarrow$82.4 & 51.1$\rightarrow$46.8 \\
log-mel, G-trained & 72.4$\rightarrow$75.7 & 30.6$\rightarrow$33.1 \\
BC-ResNet-3 log-mel & 76.5$\rightarrow$75.1 & 33.8$\rightarrow$31.3 \\
BC-ResNet-3 \nfn & 78.8$\rightarrow$77.0 & 47.1$\rightarrow$40.5 \\%

